FourierKAN outperforms MLP on Text Classification Head Fine-tuning

In resource constraint settings, adaptation to downstream classification tasks involves fine-tuning the final layer of a classifier (i.e. classification head) while keeping rest of the model weights frozen. Multi-Layer Perceptron (MLP) heads fine-tuned with pre-trained transformer backbones have long been the de facto standard for text classification head fine-tuning. However, the fixed non-linearity of MLPs often struggles to fully capture the nuances of contextual embeddings produced by pre-trained models, while also being computationally expensive. In our work, we investigate the efficacy of KAN and its variant, Fourier KAN (FR-KAN), as alternative text classification heads. Our experiments reveal that FR-KAN significantly outperforms MLPs with an average improvement of 10% in accuracy and 11% in F1-score across seven pre-trained transformer models and four text classification tasks. Beyond performance gains, FR-KAN is more computationally efficient and trains faster with fewer parameters. These results underscore the potential of FR-KAN to serve as a lightweight classification head, with broader implications for advancing other Natural Language Processing (NLP) tasks.

==> tabAblation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\definecolor{lightblue}{rgb}{0.9, 0.95, 1.0}
\definecolor{mygreen}{rgb}{0.01, 0.5, 0.01}
\definecolor{myred}{rgb}{0.8, 0.01, 0.01}

\begin{table*}[ht!]

\centering
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\textbf{Dataset}             & \textbf{Classifier} & \textbf{\#PC(k) \textcolor{myred}{$\downarrow$}} & \textbf{Acc \textcolor{mygreen}{$\uparrow$}} & \textbf{F1 \textcolor{mygreen}{$\uparrow$}} \\ \midrule
\multirow{3}{*}{AgNews}  & MLP-40              & 30.9                  & 0.835        & 0.831       \\ 
& KAN-1 & 30.7 &0.812	& 0.813  \\ 
&\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}30.7                  &\cellcolor{lightblue}\textbf{0.877}        &\cellcolor{lightblue}\textbf{0.876}       \\

       & Diff                & \textcolor{mygreen}{-0.2}                   & \textcolor{mygreen}{+0.04}        &  \textcolor{mygreen}{+0.05}       \\ \midrule
\multirow{3}{*}{Dbpedia}                           
                         & MLP-138             & 108.1                 & 0.892        & 0.891       \\ 
                         &KAN-1&107.5&0.843&0.842\\
                          &\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}107.5                 & \cellcolor{lightblue}\textbf{0.970}        &\cellcolor{lightblue}\textbf{0.971}       \\
                         & Diff                & \textcolor{mygreen}{-0.6}                     &  \textcolor{mygreen}{+0.08}        &  \textcolor{mygreen}{+0.08}       \\ \midrule
\multirow{3}{*}{IMDb}                                
                         & MLP-20              & 15.4                  & 0.778        & 0.777       \\ 
                         & KAN-1 & 15.4 & 0.739 &0.739\\
                         &\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}15.4                  & \cellcolor{lightblue}\textbf{0.831}        &\cellcolor{lightblue}\textbf{0.830}       \\
                         & Diff                & 0.0                   &  \textcolor{mygreen}{+0.05}        &  \textcolor{mygreen}{+0.05}      \\ \midrule 
\multirow{3}{*}{Papluca}                             
                         & MLP-196             & 154.6                 & 0.816        & 0.819       \\ 
                         & KAN-1 & 153.6 & 0.730 & 0.733\\
                          & \cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}153.6                 &\cellcolor{lightblue}\textbf{0.986}        &\cellcolor{lightblue}\textbf{0.986}       \\
                         & Diff                & \textcolor{mygreen}{-1.0}                     &  \textcolor{mygreen}{+0.17}        & \textcolor{mygreen}{+0.17}      \\ \midrule
\multirow{3}{*}{SST-5}        
                         & MLP-50              & 38.7                  & 0.351        & 0.176       \\ 
                         & KAN-1 & 38.4 & 0.307 & 0.231\\
                          &\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}38.4                  &\cellcolor{lightblue}\textbf{0.401}        &\cellcolor{lightblue}\textbf{0.336}       \\
                         & Diff                & \textcolor{mygreen}{-0.3}                    & \textcolor{mygreen}{+0.05}       & \textcolor{mygreen}{+0.16 }       \\ \midrule
\multirow{3}{*}{TREC-50}          
                         & MLP-477             & 512.8                 & 0.179        & 0.006       \\ 
                         & KAN-1 & 384 & 0.188	& 0.017 \\
                         &\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}384                   & \cellcolor{lightblue}\textbf{0.351}        &\cellcolor{lightblue}\textbf{0.057}       \\
                         & Diff                & \textcolor{mygreen}{-0.8}                    & \textcolor{mygreen}{+0.17}        & \textcolor{mygreen}{+0.05 }       \\ \midrule
\multirow{3}{*}{YELP-Full}     
                         & MLP-50              & 38.7                  & 0.458        & 0.456       \\ 
                         & KAN-1 & 38.4 & 0.338 & 0.324\\
                         &\cellcolor{lightblue}FR-KAN-5               &\cellcolor{lightblue}38.4                  &\cellcolor{lightblue}\textbf{0.492}        &\cellcolor{lightblue}\textbf{0.475}       \\
                         & Diff                & \textcolor{mygreen}{-0.3}                     & \textcolor{mygreen}{+0.03}        &\textcolor{mygreen}{+0.02}       \\ \bottomrule
\end{tabular}%
}
\caption{Parameter count, accuracy, and F1 score of DistilBERT using different classification heads across all datasets. MLP-$x$ represents a 2-layer perceptron with $x$ hidden layer width. KAN-$x$ and FR-KAN-$x$ represent the corresponding 1-layer network with grid size $x$. The differences between the FR-KAN head and MLP have been shown.}
\label{tab:performanceParameters}
\end{table*}
